Multi-Modal Conformal Prediction Regions with Simple Structures by Optimizing Convex Shape Templates

Conformal prediction is a statistical tool for producing prediction regions for machine learning models that are valid with high probability. A key component of conformal prediction algorithms is a \emph{non-conformity score function} that quantifies how different a model's prediction is from the unknown ground truth value. Essentially, these functions determine the shape and the size of the conformal prediction regions. While prior work has gone into creating score functions that produce multi-model prediction regions, such regions are generally too complex for use in downstream planning and control problems. We propose a method that optimizes parameterized \emph{shape template functions} over calibration data, which results in non-conformity score functions that produce prediction regions with minimum volume. Our approach results in prediction regions that are \emph{multi-modal}, so they can properly capture residuals of distributions that have multiple modes, and \emph{practical}, so each region is convex and can be easily incorporated into downstream tasks, such as a motion planner using conformal prediction regions. Our method applies to general supervised learning tasks, while we illustrate its use in time-series prediction. We provide a toolbox and present illustrative case studies of F16 fighter jets and autonomous vehicles, showing an up to $68\%$ reduction in prediction region area compared to a circular baseline region.

==> 40shapeTemplates.tex <==
\subsection{Types of Parameterized Shape Templates}
\label{sec:shapeTemplateExamples}

\subsubsection{Ellipsoidal Template}
\label{sec:shapeTemplateEllipse}

The definition for an ellipse in $\mathbb{R}^n$, denoted as Ell, parameterized by $\theta=\{ Q \succ 0 \in \mathbb{R}^{n\times n}, c \in \mathbb{R}^n\}$ is

\begin{equation}
    \text{Ell}_\theta \coloneqq \{ z \in \mathbb{R}^n | (z-c)^T Q (z-c) \leq 1 \}
\end{equation}


To convert this into the format required by~\Cref{sec:shapeConstruction}, note that 

\begin{equation}
    z \in Ell_\theta \iff (z-c)^T Q (z-c) - 1 \leq 0
\end{equation}

So the shape template for an ellipse is

\begin{equation}
     f_{\theta}(z)= (z-c)^T Q (z-c) - 1
\end{equation}

We optimize this shape during the fitting stage by utilizing CMA-ES, a genetic algorithm \cite{hansen_reducing_2003,hansen_cma-espycma_2023}. This approach finds the matrix $Q$, and center point $c$ that solves the problem \Cref{eq:ellipse_optim}.

\begin{mini}
        {Q,c}
        {\pi/\sqrt{\text{det}(Q)}}
        {\label{eq:ellipse_optim}}  
        {}
        \addConstraint{(z-c)^T Q (z-c)}{\leq 1}{\, \forall z \in Z_i}
\end{mini}

\subsubsection{Convex Hull Template}
The definition for a Convex Hull template in $\mathbb{R}^n$, denoted $\textrm{CXH}$ is parameterized by $\theta = \{A \in \mathbb{R}^{k\times n}, b\in \mathbb{R}^k\}$ is:
\begin{equation}
    \textrm{CXH}_\theta = \left\{z \in \mathbb{R}^n | Ax - b \leq 0 \right\}
\end{equation}
where $k$ is the number of facets in the Convex Hull. To convert this to a format compatible with \Cref{sec:shapeConstruction}, we first notice that an item is in the set if and only if $Ax-b$ for every term is less than $0$. We therefore define the shape template as:
\begin{equation}
    f_\theta(z) = \max_{i\in \{1,\ldots, k\}} A_{i} x -b_i
\end{equation}
where $A_i$ and $b_i$ denote the $i^{th}$ rows of $A$ and $b$, respectively.

This shape is fit using the Quickhull Algorithm \cite{barber_quickhull_1996}, which generates a convex polytope that contains all of the points in $Z_i$.

%If all of the values are less than zero, then the value of this function will also be less than zero, preserving the property that values less than zero represent items inside the shape. For any item outside the shape, one of the values will be above zero, and the shape template function will also be above zero.

\subsubsection{Hyper-Rectangle Template}
Our shape template for hyper-rectangles is fairly simple, as it does not skew the orientation of the hyper-rectangles. The template is parametrized by $\theta = \{b_{min} \in \mathbb{R}^n, b_{max} \in \mathbb{R}^n\}$. The definition for a Hyper-rectangular template $\textrm{HypRect}$ is given below:

\begin{equation}
    \textrm{HypRect}_\theta = \left\{ z\in \mathbb{R}^n | b_{min} \leq z \leq b_{max} \right\}
\end{equation}

The shape template function that we generate to comply with \Cref{sec:shapeConstruction} is based on the observation that a point contained in the hyperrectangle must satisfy the condition in \Cref{eq:hyp_rect_obs}, that each value of $z$ in each dimension should be less than $b_{min}$, and less than $b_{max}$.

\begin{equation}
    \label{eq:hyp_rect_obs}
    z \in \textrm{HypRect}_\theta \iff \max_{i\in \{1,\ldots, n\}} \max \left\{ b_{min,i} - z_i, z_i - b_{max,i} \right\} \leq 0
\end{equation}

This observation directly yields our shape template function:

\begin{equation}
    f_\theta(z) = \max_{i\in \{1,\ldots, n\}} \max \left\{ b_{min,i} - z_i, z_i - b_{max,i} \right\}
\end{equation}

This shape is fit by simply finding the element-wise minimum and maximum of the datapoints in $Z_i$.



==> archive_approach.tex <==

We first have to set up some notation. Let us denote the elements of the first calibration dataset as $D_{cal,1}:=\{Y^{(1)},\hdots,Y^{(n_1)}\}$ where $n_1>0$ is the size of the first calibration dataset. Recall that each element $Y^{(i)}$ of $D_{cal,1}$ is defined as $Y^{(i)}=(Y_{T_{obs}}^{(i)},\hdots,Y_0^{(i)},Y^{(i)}_1,\hdots,Y^{(i)}_T)$. Using the trajectory predictor $h$, we obtain predictions  $(\hat{Y}_1^{(i)},\hdots,\hat{Y}_T^{(i)})$ for $(Y^{(i)}_1,\hdots,Y^{(i)}_T)$ as per equation \eqref{eq:predi}.

We then compute the prediction error $R_{t}^{(i)}$ according to equation \eqref{eq:RfuncL2} for each calibration trajectory and for each time step, i.e., for each $t\in\{1,\hdots,T\}$ and $i\in\{1,\hdots,n_1\}$. More formally,  we compute for each calibration trajectory
\begin{align}\label{eq:non_pred_err}
    R_t^{(i)}:=R_p(Y_t^{(i)},\hat{Y}_t^{(i)}).
\end{align}

%\textcolor{red}{These $R_t^{(i)}$ values are still undefined, i.e., $R_t^{(i)}:=\|Y_t^{(i)}-\hat{Y}_t^{(i)}\|$. I think it would make the most sense to define them after equation (2).}

We can now cast the problem of finding the parameters $\alpha_1,\hdots,\alpha_T$  as the following optimization problem.

\begin{subequations}\label{eq:highLevelOptimization_}
\begin{align} 
    \min_{ \alpha_1,\hdots,\alpha_T} &\quad \text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)}, \infty \},1-\delta) \label{eq:highLevelOptimization} \\
    \text{s.t.} & \quad R^{(i)} = \text{max}(\alpha_1 R^{(i)}_1, \hdots, \alpha_T R^{(i)}_T), i=1,\hdots,n_1 \label{eq:highLevelOptimizationb}  \\
    & \quad \sum_{j=1}^{T} \alpha_j = 1 \label{eq:highLevelOptimizationc}  \\
    & \quad \alpha_j > 0, j=1,\hdots,T \label{eq:highLevelOptimizationd}
\end{align}
\end{subequations}
where we recall that $\text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)}, \infty \},1-\delta)$ denotes the empirical $1-\delta$ quantile of the set $\{ R^{(1)}, \hdots, R^{(n_1)}, \infty \}$. \Cref{eq:highLevelOptimizationc,eq:highLevelOptimizationd} normalize $\alpha_1,\hdots,\alpha_T$ and ensure them to be positive. 

\begin{remark}
    We note that the optimization problem in equation \eqref{eq:highLevelOptimization_} is always feasible. This follows since any set of parameters $\alpha_1,\hdots,\alpha_T$ that satisfy \Cref{eq:highLevelOptimizationc,eq:highLevelOptimizationd} constitute a feasible solution to \eqref{eq:highLevelOptimization_}.
\end{remark}

%\textcolor{red}{Add remark about this problem always being feasible.}

To solve the optimization problem in equation \eqref{eq:highLevelOptimization_}, we transform it into a linear complementarity program \cite{cottle2009linear} that has the same optimal value as \eqref{eq:highLevelOptimization_}. To do so, we first reformulate the $\text{max}()$ operator in equation \eqref{eq:highLevelOptimizationb} as a set of mixed integer linear program (MILP) constraints, which we then {transform} into a set of linear program constraints. We show that this transformation preserves the optimal value of \eqref{eq:highLevelOptimization_} (see Section \ref{sec:maxFormulation}). Then, we reformulate the Quantile function from equation \eqref{eq:highLevelOptimization} into a linear program (LP) that we further reformulate using its KKT conditions (see Section \ref{sec:quantileKKT}), resulting in a linear complementarity program.


\subsection{Reformulating the Max Operator}
\label{sec:maxFormulation}

%\textcolor{red}{Cite MPC for STL paper for MILP max encoding: https://arxiv.org/abs/1703.09563 and http://cse.lab.imtlucca.it/~bemporad/publications/papers/automatica-mld.pdf}

We first use ideas from \cite{bemporad1999,raman2014model} for encoding the max operator in \eqref{eq:highLevelOptimizationb} as an MILP. Therefore, we introduce the binary variables $b_t^{(i)}\in \{ 0,1\}$ for each time $t\in\{1,\hdots,T\}$ and calibration trajectory $i\in\{1,\hdots,n_1\}$. The equality constraint $R^{(i)} = \text{max}(\alpha_1 R_1^{(i)}, \hdots, \alpha_T R_T^{(i)})$ in equation \eqref{eq:highLevelOptimizationb} is then equivalent to the following MILP constraints:
\begin{subequations} \label{eq:maxConstraints}
\begin{align}
    & \quad R^{(i)} \geq \alpha_t R_t^{(i)}, \; t=1,\hdots,T \\
    & \quad R^{(i)} \leq \alpha_t R_t^{(i)} + (1-b_t^{(i)}) M, \; t=1,\hdots,T  \\
    & \quad \sum_{t=1}^{T} b_t^{(i)} = 1  \\
    & \quad b_t^{(i)} \in \{ 0,1\}, \; t=1,\hdots,T 
\end{align}
\end{subequations}
where $M>0$ is a sufficiently large and positive constant.\footnote{See \cite{bemporad1999} for the exact conditions required of $M$.}

By replacing the max operator in \Cref{eq:highLevelOptimizationb} with the MILP encoding in \Cref{eq:maxConstraints}, we arrive at the following optimization problem:
\begin{subequations}\label{eq:highLevelOptimizationMaxMILP}
\begin{align}
    \min_{ \alpha_1,\hdots,\alpha_T} &\quad \text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)}, \infty \},1-\delta) \label{eq:highLevelOptimizationMaxMILPa} \\
    \text{s.t.} & \quad R^{(i)} \geq \alpha_t R_t^{(i)}, \; i=1,\hdots,n_1 \land t=1,\hdots,T \label{eq:highLevelOptimizationMaxMILPb}  \\
    %& \quad R^{(i)} \leq \alpha_t R_t^{(i)} + (1-b_t^{(i)}) M, \; t=1,\hdots,T \label{eq:highLevelOptimizationMaxMILPc}  \\
    & \quad R^{(i)} \leq \alpha_t R_t^{(i)} + (1-b_t^{(i)}) M, \; i=1,\hdots,n_1 \label{eq:highLevelOptimizationMaxMILPc}  \\ 
    & \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \; \; \land t=1,\hdots,T \nonumber  \\
    & \quad \sum_{t=1}^{T} b_t^{(i)} = 1 \label{eq:highLevelOptimizationMaxMILPd}  \\
    & \quad b_t^{(i)} \in \{ 0,1\}, \; t=1,\hdots,T \label{eq:highLevelOptimizationMaxMILPe} \\
    & \quad \eqref{eq:highLevelOptimizationc}, \; \eqref{eq:highLevelOptimizationd} \nonumber  
    %& \quad \sum_{j=1}^{T} \alpha_j = 1 \label{eq:highLevelOptimizationMaxMILPf}  \\
    %& \quad \alpha_j \geq 0, j=1,\hdots,T \label{eq:highLevelOptimizationMaxMILPg}
\end{align}
\end{subequations}
The constraints in \eqref{eq:highLevelOptimizationMaxMILP} are linear in their parameters, i.e., in $\alpha_t$, $R^{(i)}$, and $b_t^{(i)}$. The cost function in \eqref{eq:highLevelOptimizationMaxMILPa} {can be reformulated as a linear complementarity program (LCP)}, as shown in the next section. Thus, \eqref{eq:highLevelOptimizationMaxMILP} is an MILCP since the $b_t^{(i)}$ variables are binary due to equation \eqref{eq:highLevelOptimizationMaxMILPe}. Commercial solvers can solve MILCPs, but they present scalability issues for larger time horizons $T$ and calibration data $n_1$. Therefore, we present an LCP reformulation of \eqref{eq:highLevelOptimizationMaxMILP} which will achieve the same optimality in terms of the constraint function \eqref{eq:highLevelOptimizationMaxMILPa} {while providing better scalability}.

\subsubsection{Linear {complementarity relaxation} of the MILCP in \eqref{eq:highLevelOptimizationMaxMILP}}
\label{sec:relaxMax}

We start by removing the upper bound on $R^{(i)}$ in equation \eqref{eq:highLevelOptimizationMaxMILPc} and the binary variables $b_t^{(i)}$ in equations \eqref{eq:highLevelOptimizationMaxMILPd} and \eqref{eq:highLevelOptimizationMaxMILPe} from the MILCP in \eqref{eq:highLevelOptimizationMaxMILP}. This results in the optimization problem:
%Consider the following optimization problem, which we form by removing the upper bound constraint on the $R^{(i)}$ variables in the max MILP and the $b_t^{(i)}$ binary variables:
\begin{subequations} \label{eq:problemWithoutBinaryVars}
\begin{align} 
    \min_{ \alpha_1,\hdots,\alpha_T} &\quad \text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)}, \infty \},1-\delta) \label{eq:problemWithoutBinaryVarsa} \\
    \text{s.t.} & \quad R^{(i)} \geq \alpha_t R_t^{(i)}, \; i=1,\hdots,n_1 \land t=1,\hdots,T \label{eq:problemWithoutBinaryVarsb}  \\
    %& \quad R^{(i)} \leq \alpha_t R_t^{(i)} + (1-b_t^{(i)}) M, \;  i=1,\hdots,n \land t=1,\hdots,T \nonumber \\
    %& \quad \sum_{t=1}^{T} b_t^{(i)} = 1, \;  i=1,\hdots,n \nonumber \\
    & \quad \eqref{eq:highLevelOptimizationc}, \; \eqref{eq:highLevelOptimizationd} \nonumber 
\end{align}
\end{subequations}
Note that the above optimization problem is now a linear {complementarity} program due to the removal of the binary variables $b_t^{(i)}$. While the LCP in \eqref{eq:problemWithoutBinaryVars} is clearly computationally more tractable than the MILCP in \eqref{eq:highLevelOptimizationMaxMILP}, one may ask in what way the optimal solutions of these two optimization problems are related. We next prove that the optimal values (in terms of the cost functions in \eqref{eq:highLevelOptimizationMaxMILPa} and \eqref{eq:problemWithoutBinaryVarsa}) of the two optimization problems \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} are the same.

\begin{theorem}\label{thm:1}
    Let $\delta \in (0,1)$ be a failure rate and $R_t^{(i)}$ be the prediction errors as in \eqref{eq:non_pred_err} for times $t\in\{1,\hdots,T\}$ and calibration trajectories $i\in\{1,\hdots,n_1\}$ from $D_{cal,1}$. Then, the optimal {cost} values of the optimization problems \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} are equivalent.
\end{theorem}

\begin{proof}
    Assume that $\alpha_1^*,\hdots,\alpha_T^*,R^{(1),*},\hdots,R^{(n_1),*}$ is an optimal solution to the optimization problem in equation \eqref{eq:problemWithoutBinaryVars}. We will first show that we can use $\alpha_1^*,\hdots,\alpha_T^*,R^{(1),*},\hdots,R^{(n_1),*}$ to construct a feasible solution to the optimization problem in \eqref{eq:highLevelOptimizationMaxMILP}, which we denote by $\bar{\alpha}_1^*,\hdots,\bar{\alpha}_T^*,\bar{R}^{(1),*},\hdots,\bar{R}^{(n_1),*}$, without altering the optimal value of the objective function. Particularly, let
    \begin{subequations}
    \begin{align}
        \bar{\alpha}_t^* &:= \alpha_t^*, \; t=1,\hdots,T \label{eq:exSolnMILPAlphas} \\
        \bar{R}^{(i),*} &:= \text{max}(\bar{\alpha}^*_1 R^{(i)}_1, \hdots, \bar{\alpha}^*_T R^{(i)}_T), \; i=1,\hdots,n_1 \label{eq:exSolnMILPRs}
    \end{align}
    \end{subequations}

    Note that there exists binary variables $\bar{b}_t^{(i)}$ along with which $\bar{\alpha}_1^*,\hdots,\bar{\alpha}_T^*,\bar{R}^{(1),*},\hdots,\bar{R}^{(n_1),*}$ are a feasible solution to the optimization problem in \eqref{eq:highLevelOptimizationMaxMILP}. This follows since \eqref{eq:exSolnMILPAlphas} satisfies \eqref{eq:highLevelOptimizationc} and \eqref{eq:highLevelOptimizationd} and \eqref{eq:exSolnMILPRs} satisfies \eqref{eq:highLevelOptimizationb} and consequently (\ref{eq:highLevelOptimizationMaxMILPb}-\ref{eq:highLevelOptimizationMaxMILPd}) for appropriate choices of $\bar{b}_t^{(i)}$ (and $M$). 

    Note specifically that $\bar{\alpha}_t^*$ and $\alpha_t^*$ are the same, while this does not necessarily hold for ${R}^{(i),*}$ and $\bar{R}^{(i),*}$. However, it is guaranteed that $\bar{R}^{(i),*} \leq R^{(i),*} \; \forall i=1,\hdots,n_1$ as the constraint in \eqref{eq:problemWithoutBinaryVarsb} ensures that $R^{(i),*}$ is lower bounded by $\text{max}(\alpha^*_1 R^{(i)}_1, \hdots, \alpha^*_T R^{(i)}_T)=\text{max}(\bar{\alpha}^*_1 R^{(i)}_1, \hdots, \bar{\alpha}^*_T R^{(i)}_T)$. Since the Quantile function is a monotone operator (its value is non-increasing if inputs are non-increasing), the value of the objective function in \eqref{eq:highLevelOptimizationMaxMILP} that corresponds to $\bar{\alpha}_1^*,\hdots,\bar{\alpha}_T^*,\hdots,\bar{R}^{(1),*},\bar{R}^{(n_1),*}$ can not be greater than the value of the objective function in \eqref{eq:problemWithoutBinaryVars} that corresponds to $\alpha_1^*,\hdots,\alpha_T^*,R^{(1),*},\hdots,R^{(n_1),*}$. 
    %So the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} (in terms of the objective function value) cannot be less than the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} because we can always project the the solution of Problem \eqref{eq:problemWithoutBinaryVars} onto the feasible set of solutions to Problem \eqref{eq:highLevelOptimizationMaxMILP} without increasing the value of the objective function. 
    %So the $\alpha_1^*,\hdots,\alpha_T^*$ values are not affected by the projection and the $R^{(1),*},\hdots,R^{(T),*}$ values can only be decreased or unchanged (i.e. not increased) by the projection. That means the objective function value will not increase, since the Quantile function value does not increase if its inputs are decreased or held constant. So the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} (in terms of the objective function value) cannot be less than the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} because we can always project the the solution of Problem \eqref{eq:problemWithoutBinaryVars} onto the feasible set of solutions to Problem \eqref{eq:highLevelOptimizationMaxMILP} without increasing the value of the objective function. 





    
    %The first step is to project $\alpha_1^*,\hdots,\alpha_T^*,R^{(1),*},R^{(T),*}$ onto the set of feasible values for Problem \eqref{eq:highLevelOptimizationMaxMILP}.



    %First, note that because we are only removing constraints from the problem, the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} is guaranteed to be at least as good as the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} with respect to the objective function value.

    
    
    %Consider the following method for projecting $\alpha_1^*,\hdots,\alpha_T^*,R^{(1),*},R^{(T),*}$ onto the set of feasible values for Problem \eqref{eq:highLevelOptimizationMaxMILP}:
    %\begin{subequations}
    %\begin{align}
    %    \text{proj}(\alpha_i^*) &= \alpha^*_i \\
    %    \text{proj}(R^{(i),*}) &= \text{max}(\alpha^*_1 R^{(i)}_1, \hdots, \alpha^*_T R^{(i)}_T)
    %\end{align}
    %\end{subequations}
    
    %The projection leaves the $\alpha_1^*,\hdots,\alpha_T^*$ values unchanged, since the constraints of their values are the same for both problems. It is guaranteed that $\text{proj}(R^{(i),*}) \leq R^{(i),*}$, since constraint \eqref{eq:problemWithoutBinaryVarsb} in Problem \eqref{eq:problemWithoutBinaryVars} ensures that $R^{(i),*}$ is lower bounded by $\text{max}(\alpha^*_1 R^{(i),*}_1, \hdots, \alpha^*_T R^{(i),*}_T)$. So the $\alpha_1^*,\hdots,\alpha_T^*$ values are not affected by the projection and the $R^{(1),*},\hdots,R^{(T),*}$ values can only be decreased or unchanged (i.e. not increased) by the projection. That means the objective function value will not increase, since the Quantile function value does not increase if its inputs are decreased or held constant. So the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} (in terms of the objective function value) cannot be less than the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} because we can always project the the solution of Problem \eqref{eq:problemWithoutBinaryVars} onto the feasible set of solutions to Problem \eqref{eq:highLevelOptimizationMaxMILP} without increasing the value of the objective function.
    At the same time, we note that the optimal value of the optimization problem in \eqref{eq:problemWithoutBinaryVars} cannot be greater than the optimal value of the optimization problem in \eqref{eq:highLevelOptimizationMaxMILP} because it has strictly fewer constraints than \eqref{eq:problemWithoutBinaryVars} so that the feasible set of \eqref{eq:problemWithoutBinaryVars} contains the feasible of \eqref{eq:highLevelOptimizationMaxMILP}. As a consequence, the optimal values of \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} are equivalent.
    %Note that because we are only removing constraints from the problem, the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} is guaranteed to be at least as good as the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} with respect to the objective function value.
    %So the optimal solution to Problem \eqref{eq:problemWithoutBinaryVars} (in terms of the objective function value) cannot be greater than the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} because it has fewer constraints, but it also cannot be less than the optimal solution to Problem \eqref{eq:highLevelOptimizationMaxMILP} because we can always project the the solution of Problem \eqref{eq:problemWithoutBinaryVars} onto the feasible set of solutions to Problem \eqref{eq:highLevelOptimizationMaxMILP} without increasing the value of the objective function. Thus, the objective function values of the optimal solutions to the two problems are equivalent. %So removing the upper bound constraint and binary variables from the max MILP formulation does not affect the optimal solution to our optimization problem.
\end{proof}



%Now let's pick an $i\in [1,\hdots,n]$ and examine the corresponding $R^{(i),*}$. The constraints in the above problem guarantee that $R^{(i),*} \geq \text{max}(\alpha_1 R_1^{(i)}, \hdots, \alpha_T R_T^{(i)})$.



%Consider projecting the $\alpha_1^*,\hdots,\alpha_T^*,R^{(1)},R^{(T)}$ values onto the set of feasible values for problem (\ref{eq:highLevelOptimization}). The projection leaves the $\alpha_1^*,\hdots,\alpha_T^*$ values unchanged, since the constraints of their values are the same for both problems. For $R^{(i),*}$, the projection is as follows $$\text{proj}(R^{(i),*}) = \text{max}(\alpha^*_1 R^{(i)}_1, \hdots, \alpha^*_T R^{(i)}_T)$$
%It is guaranteed that $\text{proj}(R^{(i),*}) \leq R^{(i),*}$, since the second constraint in the relaxed problem ensures that $R^{(i)}$ is lower bounded by $\text{max}(\alpha^*_1 R^{(i)}_1, \hdots, \alpha^*_T R^{(i)}_T)$. So the $\alpha_1^*,\hdots,\alpha_T^*$ values are not affected by the projection and the $R^{(1),*},\hdots,R^{(T),*}$ values can only be decreased or unchanged (i.e. not increased) by the projection. That means the Quantile$(...)$ value will not increase, since the Quantile function value does not increase if its inputs are decreased or held constant.


%but that that projection will not affect the values of $\alpha_1^*,\hdots,\alpha_T^*$ will not raise the value of Quantile$(...)$. The $\alpha$ values are not affected by the projection because we didn't remove any constraints that affect them, while the $R^{(1),*},R^{(T),*}$ can only be decreased or held constant (i.e. not increased) by the projection, since the only constraint we removed was their upper bound constraint. That means the Quantile$(...)$ value will not increase, since the Quantile function value cannot increase if it's inputs are decreased or held constant.


Note that Theorem \ref{thm:1} guarantees that the optimal values of the optimization problems in \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} are equivalent. However, we do not guarantee that the optimal parameters $\alpha_1^*,\hdots,\alpha_T^*$ obtained by solving \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} will be the same as the optimization problem in \eqref{eq:highLevelOptimizationMaxMILP} may have multiple optimal solutions $\alpha_1^*,\hdots,\alpha_T^*$. Nonetheless, the linear reformulation in \eqref{eq:problemWithoutBinaryVars} is computationally tractable and cost optimal. In our experiments in \Cref{sec:alphaDiffs}, we also show that we obtain parameters from \eqref{eq:highLevelOptimizationMaxMILP} and \eqref{eq:problemWithoutBinaryVars} that are almost equivalent. 



%Thus every solution to the relaxed problem has an 'equivalent' solution for the original problem that has the same objective function value. Thus, removing the upper bound constraint and binary variables from the max MILP formulation does not affect the optimal solution to our optimization problem.





%$R^{(i)}$ variable in the problem. What happens to the value of the objective function?

%First off, because we are only removing a constraint, the optimal value of the objective function can only decrease. If the value of $R^{(i)}$ were increased, that would not decrease the value of the objective function, since the quantile function is monotonic. So the value of $R^{(i)}$ would remain exactly the same and the optimal value of the objective function would not change. \textcolor{red}{I need to also consider second order effects, right? Like could the value of $R^{(i)}$ increase alongside something else also changing? }

%We can repeat this argument for each $i\in [1,\hdots,n]$. Therefore, removing the upper bound constraints on the $R^{(i)}$ variables does not alter the value of the optimal solution.



\subsection{Reformulating the Quantile Function}
\label{sec:quantileKKT}

We note that the Quantile function in \eqref{eq:highLevelOptimization} can be written as the following linear program \cite{Koenker1978}:
\begin{subequations}\label{eq:quantileAsLP}
\begin{align} 
    \text{Quantile}&(\{ R^{(1)}, \hdots, R^{(n_1)} \},1-\delta) \nonumber \\ 
    = \text{argmin}_{q} &\quad \sum_{i=1}^{n_1} \left( (1-\delta) e_i^+ + \delta e_i^- \right) \label{eq:quantileAsLPa}  \\
    \text{s.t.} & \quad e_i^+-e_i^- = R^{(i)} - q, \; i=1,\hdots,n_1 \label{eq:quantileAsLPb}  \\
    & \quad e_i^+,e_i^- \geq 0, \; i=1,\hdots,n_1 \label{eq:quantileAsLPc}
\end{align}
\end{subequations}
where the optimal solution $q$ of \eqref{eq:quantileAsLP} is equivalent to $\text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)} \},1-\delta)$. However, we note that we can not directly replace $\text{Quantile}(\{ R^{(1)}, \hdots, R^{(n_1)} \},1-\delta)$ in the optimization problem in \eqref{eq:highLevelOptimization} with the linear program from equation \eqref{eq:quantileAsLP} as that would result in a problem with an objective function that is itself an optimization problem. To address this issue, we replace the optimization problem in \eqref{eq:quantileAsLP} with its KKT conditions that are as follows:
\begin{subequations} \label{eq:KKTconds}
\begin{align}
    & (1-\delta) - u_i^+ + v_i = 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsa} \\
    & \delta - u_i^- - v_i = 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsb}  \\
    & \sum_{i=1}^{n_1} v_i = 0 \label{eq:KKTcondsc}  \\
    & u_i^+ e_i^+ = 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsd}  \\
    & u_i^- e_i^- = 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondse}  \\
    & e_i^+ \geq 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsf}  \\
    & e_i^- \geq 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsg}  \\
    & e_i^+ + q - e_i^- - R^{(i)} = 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsh}  \\
    & u_i^+ \geq 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsi}  \\
    & u_i^- \geq 0, \; \; i=1,\hdots,n_1 \label{eq:KKTcondsj} 
\end{align}
\end{subequations}
Here, the constraints \eqref{eq:KKTcondsa}, \eqref{eq:KKTcondsb} and \eqref{eq:KKTcondsc} encode the stationarity condition, the constraints \eqref{eq:KKTcondsd} and \eqref{eq:KKTcondse} encode complementary slackness, the constraints \eqref{eq:KKTcondsf}, \eqref{eq:KKTcondsg}, and \eqref{eq:KKTcondsh} encode primal feasibility, and the constraints \eqref{eq:KKTcondsi} and \eqref{eq:KKTcondsj} encode dual feasibility. This is an LCP because every constraint is either linear ((\eqref{eq:KKTcondsa}-\eqref{eq:KKTcondsc}) and (\eqref{eq:KKTcondsf}-\eqref{eq:KKTcondsj})) or an equality constraint stating the multiple of two positive variables equals $0$ (\eqref{eq:KKTcondsd} and \eqref{eq:KKTcondse}).\footnote{These constraints ensure that one of the two variables equals $0$.} Despite the slight non-linearity, LCPs can be efficiently solved with existing tools \cite{yu2019solving}.

Because feasible linear optimization problems have zero duality gap \cite{bradley1977applied}, any solution to the KKT conditions in \eqref{eq:KKTconds} is also an optimal solution to Problem \eqref{eq:quantileAsLP}. %Thus we do not lose anything by replacing \Cref{eq:quantileAsLP} with it's KKT conditions. 




\subsection{Summarizing the Optimization Programs}
\label{sec:finalOptimizationProblem}

Based on the results from the previous subsections, we can formulate two optimization problems that solve \eqref{eq:highLevelOptimization_}.

First, we can exactly solve \eqref{eq:highLevelOptimization_} by replacing the max operator in \eqref{eq:highLevelOptimizationb} with the MILP in \eqref{eq:maxConstraints} and the quantile function in \eqref{eq:highLevelOptimization} with its KKT conditions in \eqref{eq:KKTconds}. The following result follows by construction (for sufficiently large $M$).
\begin{proposition}
The mixed integer linear complementarity program 
\begin{subequations}\label{eq:originalProblemMILP}
\begin{align}
    \text{min}_{q,\alpha_1,\hdots,\alpha_T} &\quad q \\
    \text{s.t.} & \quad \eqref{eq:highLevelOptimizationMaxMILPb}, \; \eqref{eq:highLevelOptimizationMaxMILPc}, \; \eqref{eq:highLevelOptimizationMaxMILPd}, \; \eqref{eq:highLevelOptimizationMaxMILPe} \nonumber \\
    & \quad \eqref{eq:KKTcondsa}, \; \eqref{eq:KKTcondsb}, \; \eqref{eq:KKTcondsc}, \; \eqref{eq:KKTcondsd}, \; \eqref{eq:KKTcondse} \nonumber \\ 
    & \quad \eqref{eq:KKTcondsf}, \; \eqref{eq:KKTcondsg}, \; \eqref{eq:KKTcondsh}, \; \eqref{eq:KKTcondsi}, \; \eqref{eq:KKTcondsj}  \nonumber \\
    & \quad \eqref{eq:highLevelOptimizationc}, \; \eqref{eq:highLevelOptimizationd} \nonumber  
    %& \quad  R^{(i)} \geq \alpha_t R_t^{(i)}, \; i=1,\hdots,n \land t=1,\hdots,T  \\
    %& \quad R^{(i)} \leq \alpha_t R_t^{(i)} + (1-b_t^{(i)}) M, \; i=1,\hdots,n  \\ 
    %& \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \land t=1,\hdots,T \nonumber  \\
    %& \quad b_t^{(i)} \in [0,1], \; \; \forall i=1,\hdots,n \land t=1,\hdots,T  \\
    %& \quad \sum_{t=1}^{T} b_t^{(i)} = 1, \;  i=1,\hdots,n  \\
    %& \quad \eqref{eq:highLevelOptimizationc}, \; \eqref{eq:highLevelOptimizationd} \nonumber \\
    %& \quad (1-\delta) + u_i^+ + v_i = 0, \; \; i=1,\hdots,n  \\
    %& \quad \delta + u_i^- - v_i = 0, \; \; i=1,\hdots,n  \\
    %& \quad \sum_i v_i = 0  \\
    %& \quad u_i^+ e_i^+ = 0, \; u_i^- e_i^- = 0, \; \; i=1,\hdots,n  \\
    %& \quad e_i^+ \geq 0, \; e_i^- \geq 0, \; \; i=1,\hdots,n  \\
    %& \quad e_i^+ + q - e_i^- - R^{(i)} = 0, \; \; i=1,\hdots,n  \\
    %& \quad u_i^+ \geq 0, \; u_i^- \geq 0, \; \; i=1,\hdots,n 
\end{align}
is equivalent to the optimization problem in \eqref{eq:highLevelOptimization_}.
\end{subequations}
\end{proposition}

Second, by further removing the upper bound from the max operator as described in \Cref{sec:relaxMax}, we can solve a linear complementarity program that has the same optimal {cost} value as \eqref{eq:highLevelOptimization_}. This result follows from Theorem \ref{thm:2}.
\begin{proposition}
The linear complementarity program
\begin{subequations}\label{eq:relaxedProblemLP}
\begin{align}
    \text{min}_{q,\alpha_1,\hdots,\alpha_T} &\quad q \\
    \text{s.t.} & \quad \eqref{eq:highLevelOptimizationMaxMILPb} \nonumber \\
    & \quad \eqref{eq:KKTcondsa}, \; \eqref{eq:KKTcondsb}, \; \eqref{eq:KKTcondsc}, \; \eqref{eq:KKTcondsd}, \; \eqref{eq:KKTcondse} \nonumber \\ 
    & \quad \eqref{eq:KKTcondsf}, \; \eqref{eq:KKTcondsg}, \; \eqref{eq:KKTcondsh}, \; \eqref{eq:KKTcondsi}, \; \eqref{eq:KKTcondsj}  \nonumber \\
    & \quad \eqref{eq:highLevelOptimizationc}, \; \eqref{eq:highLevelOptimizationd} \nonumber  
\end{align}
\end{subequations}
has the same optimal value as the optimization problem  \eqref{eq:highLevelOptimization_}.
\end{proposition}


%The first line of constraints encodes the relaxed $R^{(i)} = \text{max}(\alpha_1 R^{(i)}_1, \hdots, \alpha_T R^{(i)}_T)$ constraint from \Cref{sec:maxFormulation}, the next two are copied directly from \Cref{eq:highLevelOptimization}, and the last 10 are the KKT conditions for the quantile computation from \Cref{sec:quantileKKT}.






\section{Conformal Prediction Regions for Time-Series}
\label{sec:second_approach}

Finally, after obtaining the parameters $\alpha_1,\hdots,\alpha_T$ from the first calibration dataset $D_{cal,1}$ by solving \eqref{eq:originalProblemMILP} or \eqref{eq:relaxedProblemLP}, we can apply conformal prediction with the non-conformity score $R$ as defined in \eqref{eq:generalRfunc} to obtain prediction regions for time series. We do so by following  \Cref{sec:intro_cp} and using the second calibration dataset $D_{cal,2}$. 



More formally, let us denote the elements of the second calibration dataset as $D_{cal,2}:=\{Y^{(n_1+1)},\hdots,Y^{(n)}\}$ where $n-n_1>0$ is the size of the second calibration dataset.\footnote{Recall the $n$ is the size of $D_{cal}$ and $n_1$ is the size of $D_{cal,1}$.} For each calibration trajectory $i\in\{n_1+1,\hdots,n\}$, we compute the nonconformity score as
\begin{align}\label{eq:cal_R_}
    R^{(i)}:=\max\left(\alpha_1 R_p(Y_1^{(i)}, \hat{Y}_1^{(i)}), \hdots, \alpha_T R_p(Y_T^{(i)},\hat{Y}_T^{(i)})\right).
\end{align}
We are now ready to state the final result of our paper in which we obtain prediction regions for $R:=\max\left(\alpha_1 R_p(y_1, \hat{y}_1), \hdots, \alpha_T R_p(y_T,\hat{y}_T)\right)$.
\begin{theorem}\label{thm:2}
Let $Y$ be a trajectory drawn from $\mathcal{D}$ and let $\hat{Y}=h(Y_{T_{obs}},\hdots,Y_0)$ be predictions from the time series predictor $h$. Let $\delta \in (0,1)$ be a failure rate and $R_t^{(i)}$ be the prediction error as in \eqref{eq:non_pred_err} for times $t\in\{1,\hdots,T\}$ and calibration trajectories $i\in\{1,\hdots,n_1\}$ from $D_{cal,1}$. Let $\alpha_1,\hdots,\alpha_T$ be obtained by solving \eqref{eq:originalProblemMILP} or \eqref{eq:relaxedProblemLP}. Further, let $R^{(i)}$ be the nonconformity score as in \eqref{eq:cal_R_} for calibration trajectories $i\in\{n_1+1,\hdots,n\}$ from $D_{cal,2}$. Finally, let $R=\max\left(\alpha_1 R_p(Y_1, \hat{Y}_1), \hdots, \alpha_T R_p(Y_T,\hat{Y}_T)\right)$. It then holds that
\begin{align}\label{eq:cpGuarantee}
    &\text{Prob}\left(R \leq C \right) \geq 1-\delta
\end{align}
where $C:=\text{Quantile}(\{ R^{(n_1+1)}, \hdots, R^{(n)} \},1-\delta)$.

\begin{proof}
    Since $\alpha_1,\hdots,\alpha_T$ are obtained from $D_{cal,1}$, the non-conformity scores $R^{(i)}$ which are computed from $D_{cal,2}$ are exchangeable. Consequently, we can apply \cite[Lemma 1]{tibshirani2019conformal} to get that \Cref{eq:cpGuarantee} holds.
\end{proof}
\end{theorem}

We point out the necessity to split the dataset $D_{cal}$ into the datasets $D_{cal,1}$ and $D_{cal,2}$ to conform to the exchangeability assumption in conformal prediction. To convert equation \eqref{eq:cpGuarantee} into practical conformal prediction regions, note that 
\begin{align*}
     R=&\text{max}\left(\alpha_1 \|Y_1-\hat{Y}_1\|,\hdots,\alpha_T \|Y_T-\hat{Y}_T\| \right)\le C \\
    \Leftrightarrow\;\;\;\;\;\;\;\; &  \|Y_t-\hat{Y}_t\|\le C/\alpha_t \; \; \forall t\in\{1,\hdots,T\}
\end{align*}

Intuitively, the conformal prediction regions provide geometric balls of radius $C/\alpha_t$ around each prediction $\hat{y}_t$ due to the use of the Euclidean norm. For an example, we refer to \Cref{fig:ORCATrace}. We remark that other choices of the prediction $R_p$ may lead to different shapes. We summarize this result next. 

\begin{corollary}
Let all conditions of Theorem \ref{thm:2} hold. Then, it follows that
    \begin{align*}
        \text{Prob}(\|Y_t-\hat{Y}_t\| \le C/\alpha_t \; \; \forall t\in\{1,\hdots,T\}) \geq 1-\delta.
    \end{align*}
\end{corollary}





==> relatedWork.tex <==
\section{Related Work}
\label{sec:relatedWork}





List of papers to mention:
\begin{itemize}
    \item our ral paper
    \item lars STL monitoring paper
    \item the other RNN CP paper
    \item our adaptive CP paper
    \item a few other adaptive CP papers
    \item one of the neural predictive monitoring papers
    \item the other stl monitoring paper that isn't as good as lars's :)
    \item 
\end{itemize}






